Probing the weak wind phenomenon in Galactic O-type giants

Analyses of Galactic late O dwarfs (O8-O9.5V) raised the `weak wind problem': spectroscopic mass loss rates ($\dot{M}$) are up to two orders of magnitude lower than the theoretical values. We investigated the stellar and wind properties of Galactic late O giants (O8-O9.5III). We performed a spectroscopic analysis of nine O8-O9.5III stars in the ultraviolet (UV) and optical regions using the model atmosphere code CMFGEN. From the UV region, we found $\dot{M}$ $\sim$ $10^{-8}-10^{-9}$ $\mathrm{M_\odot}$ $\mathrm{yr^{-1}}$ overall. This is lower by $\sim 0.9 - 2.3$ dex than the predicted values based on the (global) conservation of energy in the wind. The mass-loss rates predicted from first principles, based on the moving reversing layer theory, agree better with our findings, but it fails to match the spectroscopic $\dot{M}$ for the most luminous OB stars. The region of $\log(L_\star/L_\odot) \sim 5.2$ is critical for both sets of predictions in comparison with the spectroscopic mass-loss rates. CMFGEN models with the predicted $\dot{M}$ (the former one) fail to reproduce the UV wind lines for all the stars of our sample. We reproduce the observed H$\alpha$ profiles of four objects with our $\dot{M}$ derived from the UV. Hence, low $\dot{M}$ values (weak winds) are favored to fit the observations (UV + optical), but discrepancies between the UV and H$\alpha$ diagnostics remain for some objects. Our results indicate weak winds beyond the O8-9.5V class, since the region of $\log(L_\star/L_\odot) \sim 5.2$ is indeed critical to the weak wind phenomenon. Since O8-O9.5III stars are more evolved than O8-9.5V, evolutionary effects do not seem to play a role in the onset of the weak wind phenomenon. These findings support that the $\dot{M}$ (for low luminosity O stars) in use in the majority of modern stellar evolution codes must be severely overestimated up to the end of the H-burning phase.

==> fig_hd116852_mdot_uv_vink_uv_halpha.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5102.00,6236.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(28,3286){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(28,3861){\makebox(0,0)[r]{\strut{}$0.4$}}%
      \put(28,4437){\makebox(0,0)[r]{\strut{}$0.8$}}%
      \put(28,5012){\makebox(0,0)[r]{\strut{}$1.2$}}%
      \put(28,5587){\makebox(0,0)[r]{\strut{}$1.6$}}%
      \put(487,3046){\makebox(0,0){\strut{}$1230$}}%
      \put(1275,3046){\makebox(0,0){\strut{}$1240$}}%
      \put(2062,3046){\makebox(0,0){\strut{}$1250$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(-380,2828){\rotatebox{-270}{\makebox(0,0){\strut{}Normalized flux}}}%
      \put(1274,5875){\makebox(0,0){\strut{}\ion{N}{V} 1240}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(3091,3046){\makebox(0,0){\strut{}$1380$}}%
      \put(3642,3046){\makebox(0,0){\strut{}$1395$}}%
      \put(4193,3046){\makebox(0,0){\strut{}$1410$}}%
      \put(4744,3046){\makebox(0,0){\strut{}$1425$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3825,5875){\makebox(0,0){\strut{}\ion{Si}{IV} 1394,1403}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(28,168){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(28,744){\makebox(0,0)[r]{\strut{}$0.4$}}%
      \put(28,1319){\makebox(0,0)[r]{\strut{}$0.8$}}%
      \put(28,1895){\makebox(0,0)[r]{\strut{}$1.2$}}%
      \put(28,2470){\makebox(0,0)[r]{\strut{}$1.6$}}%
      \put(372,-72){\makebox(0,0){\strut{}$1710$}}%
      \put(1375,-72){\makebox(0,0){\strut{}$1720$}}%
      \put(2377,-72){\makebox(0,0){\strut{}$1730$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(1274,2758){\makebox(0,0){\strut{}\ion{N}{IV} 1718}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(2846,-72){\makebox(0,0){\strut{}$6550$}}%
      \put(3458,-72){\makebox(0,0){\strut{}$6560$}}%
      \put(4071,-72){\makebox(0,0){\strut{}$6570$}}%
      \put(4683,-72){\makebox(0,0){\strut{}$6580$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(2529,-312){\makebox(0,0){\strut{}$\lambda$ (\AA)}}%
      \put(3825,2758){\makebox(0,0){\strut{}H$\alpha$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./hd116852_mdot_uv_vink_uv_halpha.pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup

